CBGL: Fast Monte Carlo Passive Global Localisation of 2D LIDAR Sensor

Navigation of a mobile robot is conditioned on the knowledge of its pose. In observer-based localisation configurations its initial pose may not be knowable in advance, leading to the need of its estimation. Solutions to the problem of global localisation are either robust against noise and environment arbitrariness but require motion and time, which may (need to) be economised on, or require minimal estimation time but assume environmental structure, may be sensitive to noise, and demand preprocessing and tuning. This article proposes a method that retains the strengths and avoids the weaknesses of the two approaches. The method leverages properties of the Cumulative Absolute Error per Ray (CAER) metric with respect to the errors of pose hypotheses of a 2D LIDAR sensor, and utilises scan--to--map-scan matching for fine(r) pose estimations. A large number of tests, in real and simulated conditions, involving disparate environments and sensor properties, illustrate that the proposed method outperforms state-of-the-art methods of both classes of solutions in terms of pose discovery rate and execution time. The source code is available for download.

==> figures/experiments/a/execution_time.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplfronttext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5000.00,1500.00)%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,264){\makebox(0,0)[r]{\strut{}\footnotesize $0.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,458){\makebox(0,0)[r]{\strut{}\footnotesize $5.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,652){\makebox(0,0)[r]{\strut{}\footnotesize $10.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,847){\makebox(0,0)[r]{\strut{}\footnotesize $15.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,1041){\makebox(0,0)[r]{\strut{}\footnotesize $20.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(990,1235){\makebox(0,0)[r]{\strut{}\footnotesize $25.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \put(0,0){\includegraphics{./figures/experiments/a/execution_time}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/experiments/a/outliers.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4000.00,2000.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,440){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,699){\makebox(0,0)[r]{\strut{}0.2}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,958){\makebox(0,0)[r]{\strut{}0.4}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,1217){\makebox(0,0)[r]{\strut{}0.6}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,1476){\makebox(0,0)[r]{\strut{}0.8}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(594,1735){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(726,220){\makebox(0,0){\strut{}0.5}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1445,220){\makebox(0,0){\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2165,220){\makebox(0,0){\strut{}1.5}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2884,220){\makebox(0,0){\strut{}2}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3603,220){\makebox(0,0){\strut{}2.5}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/media/li9i/show1/cbgl_2023_06_spell/evaluation_scripts/evaluation_scripts/ros_real/figures/outliers}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/experiments/a/xyt_errors.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(11200.00,8400.00)%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(988,840){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(988,2520){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(988,4200){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(988,5879){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(988,7559){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4269,620){\makebox(0,0){\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,840){\makebox(0,0)[r]{\strut{}$10^{-6}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,1800){\makebox(0,0)[r]{\strut{}$10^{-5}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,2760){\makebox(0,0)[r]{\strut{}$10^{-4}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,3720){\makebox(0,0)[r]{\strut{}$10^{-3}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,4679){\makebox(0,0)[r]{\strut{}$10^{-2}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,5639){\makebox(0,0)[r]{\strut{}$10^{-1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,6599){\makebox(0,0)[r]{\strut{}$10^{0}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(5748,7559){\makebox(0,0)[r]{\strut{}$10^{1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(9029,620){\makebox(0,0){\strut{}2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{/media/li9i/show1/cbgl_2023_06_spell/evaluation_scripts/evaluation_scripts/ros_real/figures/xyt_errors}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/experiments/b/exec_times.tex <==
\definecolor{c1}{RGB}{228,26,28}
\definecolor{c2}{RGB}{55,126,184}
\definecolor{c3}{RGB}{255,0,255}
\definecolor{c4}{RGB}{152,78,163}
\definecolor{c5}{RGB}{255,127,0}
\definecolor{c6}{RGB}{77,175,74}

% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplfronttext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5000.00,1500.00)%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,267){\makebox(0,0)[r]{\strut{}\footnotesize $10^{0}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,657){\makebox(0,0)[r]{\strut{}\footnotesize $10^{1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,1046){\makebox(0,0)[r]{\strut{}\footnotesize $10^{2}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(1474,-70){\makebox(0,0){\strut{}\footnotesize WAREHOUSE}}%
      \put( 400,1500){\makebox(0,0){\strut{}{\color{c1}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize MCL}}
      \put(1000,1500){\makebox(0,0){\strut{}{\color{c2}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize ALS}}
      \put(1650,1500){\makebox(0,0){\strut{}{\color{c3}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize GMCL}}
      \put(2500,1500){\makebox(0,0){\strut{}{\color{c4}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize PGL-FMIC}}
      \put(3500,1500){\makebox(0,0){\strut{}{\color{c5}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize PGL-PLICP}}
      \put(4450,1500){\makebox(0,0){\strut{}{\color{c6}{\rule[0.6mm]{0.3cm}{0.5mm}}} \scriptsize CBGL}}
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(4868,267){\makebox(0,0)[r]{\strut{}\footnotesize $10^{0}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4868,657){\makebox(0,0)[r]{\strut{}\footnotesize $10^{1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4868,1046){\makebox(0,0)[r]{\strut{}\footnotesize $10^{2}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(3524,-70){\makebox(0,0){\strut{}\footnotesize WILLOWGARAGE}}%
    }%
    \put(0,0){\includegraphics{./figures/experiments/b/exec_times}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/experiments/c/awesome.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplfronttext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(5000.00,2500.00)%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,250){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,650){\makebox(0,0)[r]{\strut{}0.2}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,1050){\makebox(0,0)[r]{\strut{}0.4}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,1449){\makebox(0,0)[r]{\strut{}0.6}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,1849){\makebox(0,0)[r]{\strut{}0.8}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(368,2249){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(826,30){\makebox(0,0){\strut{}$10^{-2}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1200,30){\makebox(0,0){\strut{}$10^{-1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1575,30){\makebox(0,0){\strut{}$10^{0}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1949,30){\makebox(0,0){\strut{}$10^{1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2323,30){\makebox(0,0){\strut{}$10^{2}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,250){\makebox(0,0)[r]{\strut{}0}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,650){\makebox(0,0)[r]{\strut{}0.2}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,1050){\makebox(0,0)[r]{\strut{}0.4}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,1449){\makebox(0,0)[r]{\strut{}0.6}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,1849){\makebox(0,0)[r]{\strut{}0.8}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2493,2249){\makebox(0,0)[r]{\strut{}1}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2813,30){\makebox(0,0){\strut{}$10^{-4}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3188,30){\makebox(0,0){\strut{}$10^{-3}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3563,30){\makebox(0,0){\strut{}$10^{-2}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3938,30){\makebox(0,0){\strut{}$10^{-1}$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4313,30){\makebox(0,0){\strut{}$10^{0}$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \put(0,0){\includegraphics{./figures/experiments/c/awesome}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/h_fig.tex <==
\definecolor{v}{RGB}{131, 186, 109}
\definecolor{x}{RGB}{217, 33, 32}
\definecolor{w}{RGB}{120, 28, 130}


% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplfronttext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4600.00,3000.00)%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,300){\makebox(0,0)[r]{\strut{}\small $0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,699){\makebox(0,0)[r]{\strut{}\small $\psi_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,1100){\makebox(0,0)[r]{\strut{}\small $400$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,1899){\makebox(0,0)[r]{\strut{}\small $800$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,2699){\makebox(0,0)[r]{\strut{}\small $1200$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(460,80){\makebox(0,0){\strut{}\small $0.05$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1378,80){\makebox(0,0){\strut{}\small $\delta_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1659,80){\makebox(0,0){\strut{}\small $1.5$}}%
      \colorrgb{0.15,0.15,0.15}%
      %\put(1903,80){\makebox(0,0){\strut{}\small $3.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2046,80){\makebox(0,0){\strut{}\small $4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      %\put(-160,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small CAER [m]}}}%
      \put(-160,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small $f_{\psi}$ [m]}}}%
      \colorrgb{0.15,0.15,0.15}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,300){\makebox(0,0)[r]{\strut{}\small $1$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,777){\makebox(0,0)[r]{\strut{}\small $10^1$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,1253){\makebox(0,0)[r]{\strut{}\small $10^2$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,1730){\makebox(0,0)[r]{\strut{}\small $10^3$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,2206){\makebox(0,0)[r]{\strut{}\small $10^4$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,2683){\makebox(0,0)[r]{\strut{}\small $10^5$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2967,80){\makebox(0,0){\strut{}\small $0.05$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3885,80){\makebox(0,0){\strut{}\small $\delta_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4166,80){\makebox(0,0){\strut{}\small $1.5$}}%
      \colorrgb{0.15,0.15,0.15}%
      %\put(4410,80){\makebox(0,0){\strut{}\small $3.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4553,80){\makebox(0,0){\strut{}\small $4.5$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      %\put(2400,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small rank in ascending CAER hierarchy}}}%
      \put(2400,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small $f_{\texttt{r}}$}}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2300,-250){\makebox(0,0){\strut{}\small estimate error \footnotesize [(m$^2$ + rad$^2$)$^{1/2}$]}}%
      \put(1300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{v}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{V}$}}}%
      \put(2300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{x}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{X}$}}}%
      \put(3300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{w}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{W}$}}}%
    }%
    \put(0,0){\includegraphics{./figures/h_fig}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/h_not_fig.tex <==
\definecolor{v}{RGB}{131, 186, 109}
\definecolor{x}{RGB}{217, 33, 32}
\definecolor{w}{RGB}{120, 28, 130}


% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplfronttext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4600.00,3000.00)%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,478){\makebox(0,0)[r]{\strut{}\small $\psi_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,1533){\makebox(0,0)[r]{\strut{}\small $500$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,2053){\makebox(0,0)[r]{\strut{}\small $1000$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(328,2573){\makebox(0,0)[r]{\strut{}\small $2000$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(460,80){\makebox(0,0){\strut{}\small $0.05$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(854,80){\makebox(0,0){\strut{}\small $5.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1251,80){\makebox(0,0){\strut{}\small $10.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(1635,80){\makebox(0,0){\strut{}\small $\delta_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2046,80){\makebox(0,0){\strut{}\small $20.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      %\put(-160,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small CAER [m]}}}%
      \put(-160,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small $f_{\psi}$ [m]}}}%
      \colorrgb{0.15,0.15,0.15}%
      %\put(1253,-250){\makebox(0,0){\strut{}\small estimate error \footnotesize [(m$^2$ + rad$^2$)$^{1/2}$]}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,300){\makebox(0,0)[r]{\strut{}\small $10^0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,700){\makebox(0,0)[r]{\strut{}\small $10^1$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,1099){\makebox(0,0)[r]{\strut{}\small $10^2$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,1499){\makebox(0,0)[r]{\strut{}\small $10^3$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,1898){\makebox(0,0)[r]{\strut{}\small $10^4$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,2298){\makebox(0,0)[r]{\strut{}\small $10^5$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2835,2698){\makebox(0,0)[r]{\strut{}\small $10^5$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2967,80){\makebox(0,0){\strut{}\small $0.05$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3361,80){\makebox(0,0){\strut{}\small $5.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(3758,80){\makebox(0,0){\strut{}\small $10.0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4142,80){\makebox(0,0){\strut{}\small $\delta_0$}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(4553,80){\makebox(0,0){\strut{}\small $20.0$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \colorrgb{0.15,0.15,0.15}%
      %\put(2400,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small rank in ascending CAER hierarchy}}}%
      \put(2400,1499){\rotatebox{90}{\makebox(0,0){\strut{}\small $f_{\texttt{r}}$}}}%
      \colorrgb{0.15,0.15,0.15}%
      \put(2300,-250){\makebox(0,0){\strut{}\small estimate error \footnotesize [(m$^2$ + rad$^2$)$^{1/2}$]}}%
      \put(1300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{v}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{V}$}}}%
      \put(2300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{x}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{X}$}}}%
      \put(3300,3000){\makebox(0,0){\makebox(0,0){\strut{}{\color{w}{\rule[0.6mm]{0.5cm}{0.75mm}}} $\mathcal{W}$}}}%
    }%
    \put(0,0){\includegraphics{./figures/h_not_fig}}%
    \gplfronttext
  \end{picture}%
\endgroup

